A Study of Variable-Role-based Feature Enrichment in Neural Models of Code

Although deep neural models substantially reduce the overhead of feature engineering, the features readily available in the inputs might significantly impact training cost and the performance of the models. In this paper, we explore the impact of an unsuperivsed feature enrichment approach based on variable roles on the performance of neural models of code. The notion of variable roles (as introduced in the works of Sajaniemi et al. [Refs. 1,2]) has been found to help students' abilities in programming. In this paper, we investigate if this notion would improve the performance of neural models of code. To the best of our knowledge, this is the first work to investigate how Sajaniemi et al.'s concept of variable roles can affect neural models of code. In particular, we enrich a source code dataset by adding the role of individual variables in the dataset programs, and thereby conduct a study on the impact of variable role enrichment in training the Code2Seq model. In addition, we shed light on some challenges and opportunities in feature enrichment for neural code intelligence models.

==> results/avg_prediction_change.tex <==
\begin{figure*}%[!htb]
    \centering
    \begin{minipage}{.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/percentage/avg_prediction_increase.pdf}
        \caption*{(a) Prediction Increase}
        \label{fig:percentage_prediction_increase}
    \end{minipage}%
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/percentage/avg_prediction_decrease.pdf}
        \caption*{(b) Prediction Decrease}
        \label{fig:percentage_prediction_decrease}
    \end{minipage}
    \caption{Percentage of average prediction change}
    \label{fig:percentage_change}
\end{figure*}


==> results/max_probability_change.tex <==
\begin{figure*}%[!htb]
    \centering
    \begin{minipage}{.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/percentage/max_probability_increase.pdf}
        \caption*{(a) Probability Increase}
    \end{minipage}%
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/percentage/max_probability_decrease.pdf}
        \caption*{(b) Probability Decrease}
    \end{minipage}
    \caption{Maximum probability change over target samples.}
    \label{fig:max_probability_change}
\end{figure*}


==> results/summary_all.tex <==

\begin{table*}%[!htb]
    \caption{Summary of average probability change (the average change of probability score during reduction steps for a sample).}
    \label{table:summary_probability_change}
    \def\arraystretch{1.2}
    
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|r|r|r|c|r|r|r|}
        \hline
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{4}{c|}{Probability Increase ($+\Delta{s}$)}
        & \multicolumn{4}{c|}{Probability Decrease ($-\Delta{s}$)}
        \\ \cline{3-10}
        &
        & \textbf{Sample($\%$)} & \textbf{Min} & \textbf{Max} & \textbf{Avg}
        & \textbf{Sample($\%$)} & \textbf{Min} & \textbf{Max} & \textbf{Avg}
        \\ \hline 
        \hline
        
        \multirow{2}{*}{\sbabi} & \rnn 
        & 97.80 & 0.01 & 42.80 & 6.75
        & 100.00 & -0.06 & -46.07 & -4.81
        \\ \cline{2-10}
        
        & \cnn 
        & 90.70 & 0.01 & 48.77 & 5.86
        & 100.00 & -0.02 & -44.49 & -6.64
        \\ \hline
        
        \multirow{2}{*}{\jlarge} & \ctv 
        & 91.70 & 0.01 & 50.12 & 5.20
        & 95.80 & -0.01 & -72.38 & -7.57
        \\ \cline{2-10}
        
        & \cts 
        & 97.10 & 0.01 & 54.56 & 4.55
        & 99.90 & -0.01 & -65.36 & -6.30
        \\ \hline
        
        \multirow{2}{*}{\pyg} & \rnn 
        & 99.50 & 0.01 & 44.80 & 8.29
        & 100.00 & -0.01 & -36.11 & -9.15
        \\ \cline{2-10}
        
        & \tra 
        & 98.20 & 0.01 & 45.80 & 8.31
        & 100.00 & -0.01 & -44.68 & -9.59
        \\ \hline
        
    \end{tabular}%
    }
\end{table*}


==> results/summary_probability_change.tex <==

\begin{table*}%[!htb]
    \caption{Summary of average probability change (when the change of probability score is more than 0.1 during reduction steps for a sample).}
    % Fixed - \TODO{It's not 0.42\% but 42\%? of the samples, right?}
    \label{table:summary_probability_change}
    \def\arraystretch{1.2}
    
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|r|r|r|c|r|r|r|}
        \hline
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{4}{c|}{Probability Increase ($+\Delta{s}$)}
        & \multicolumn{4}{c|}{Probability Decrease ($-\Delta{s}$)}
        \\ \cline{3-10}
        &
        & \textbf{Sample($\%$)} & \textbf{Min} & \textbf{Max} & \textbf{Avg}
        & \textbf{Sample($\%$)} & \textbf{Min} & \textbf{Max} & \textbf{Avg}
        \\ \hline 
        \hline
        
        \multirow{2}{*}{\sbabi} & \rnn 
        & 42.10 & 0.10 & 0.48 & 0.20
        & 43.50 & -0.10 & -0.48 & -0.19
        \\ \cline{2-10}
        
        & \cnn 
        & 32.20 & 0.10 & 0.49 & 0.23
        & 54.00 & -0.10 & -0.50 & -0.24
        \\ \hline
        
        \multirow{2}{*}{\jlarge} & \ctv 
        & 46.20 & 0.10 & 0.72 & 0.25
        & 64.10 & -0.10 & -0.74 & -0.27
        \\ \cline{2-10}
        
        & \cts 
        & 44.90 & 0.10 & 0.55 & 0.18
        & 72.70 & -0.10 & -0.69 & -0.22
        \\ \hline
        
        \multirow{2}{*}{\pyg} & \rnn 
        & 85.00 & 0.10 & 0.45 & 0.22
        & 93.50 & -0.10 & -0.64 & -0.24
        \\ \cline{2-10}
        
        & \tra 
        & 79.80 & 0.10 & 0.59 & 0.22
        & 95.30 & -0.10 & -0.60 & -0.23
        \\ \hline
        
    \end{tabular}%
    }
\end{table*}


==> results/top_reduced_tokens.tex <==

\begin{table*}%[!htb]
    \caption{Top 15 distractor tokens in reduction steps where model's prediction probability score changes by at least $0.1$ ($+\Delta{s}$ = probability increase and $-\Delta{s}$ = probability decrease) \TODO{Group by categories}.}
    \label{table:top_reduction_tokens}
    \def\arraystretch{1.2}
    
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Task} & \textbf{Probability Change} & \textbf{Top 15 Tokens (separated by space)} \\ \hline 
        \hline
        
        \multirow{2}{*}{\vd} & $+\Delta{s}$ &
        ; VARIABLE = int char 0 NUMBER if else rand $<$ return for ++ while \\ \cline{2-3}
        & $-\Delta{s}$ &
        VARIABLE ; = char int if NUMBER $<$ rand 0 for return else ++ while \\ \hline

        \multirow{2}{*}{\vm} & $+\Delta{s}$ &
        NEWLINE . = INDENT : UNINDENT return if in None for assertEqual == \% 1 \\ \cline{2-3}
        & $-\Delta{s}$ &
        NEWLINE . = : INDENT UNINDENT if return None for assertEqual in def \_\_init\_\_ 1 \\ \hline

        \multirow{2}{*}{\mn} & $+\Delta{s}$ & 
        ; . = return if nan super new : ! 0 1 + uri this \\ \cline{2-3}
        & $-\Delta{s}$ &
        . ; return = super if Override $@$ new this ! nan : 0 qname\\ \hline
        
    \end{tabular}%
    }
\end{table*}


==> sections/settings.tex <==
\section{Experimental Settings}
\label{sec-set}

In this section, we elaborate on our training environment, describe the model trained, and the datasets used to train the model in Subsections~\ref{subsec-setup}, \ref{subsec-subj-model}, and \ref{subsec-train}. Finally, in Subsection~\ref{subsec-eval}, we present details of the test sets used to evaluate the generated trained models.

\subsection{Training Environment}
\label{subsec-setup}
For training \cts with the original and the augmented datasets, we used a system with a 12GB NVIDIA GPU and 12 Intel 2.30GHz CPUs, and a system with a 24GB NVIDIA GPU and 64 Intel 2.90GHz CPUs. We used a training batch size of 256 samples for all the training sessions, and the default settings for the remaining parameters as per the \cts repository.  
%We used a system with a 12GB NVIDIA GPU and 12 Intel 2.30GHz CPUs, and a system with a 24GB NVIDIA GPU and 64 Intel 2.90GHz CPUs to train \cts with \JL and \JLR respectively. 

%We trained \cts with \JL for 52 epochs, and with \JLR for 28 epochs. 
%In total, we spent about 11 and a half days of GPU cycles towards training the models. 
%In total, we spent around 20 days of GPU cycles towards training the models. 

%DONE \bowen{maybe it's better to mention all the test datasets for both Performance and Robustness under this section and describe them into two separate subsubsections here.}

%The test sets do not overlap with the train sets, and thus consist of unseen data.

%DONE \bowen{move the corresponding content here}

\begin{comment}
\begin{itemize}[leftmargin=*]
    \item \JLT Test Set -- This is a semantically-transformed test set created in~\cite{rabin2021generalizability}, from the \JL dataset, which consists of 916,611 methods, where a random number of variables in the entire dataset where renamed.
    \item \JLTR Test Set -- We generate this test set from the \JLT Test Set above, by augmenting variables with roles information. 
\end{itemize}
\end{comment}

%Addressed --> \bowen{maybe it's more friendly to just move the content in Section 3.2 to this section rather ask reviewers to read back to 3.2} --> added note on this in section 3.2






